Measurements of $\pi^\pm$, K$^\pm$, p and $\bar{\textrm{p}}$ spectra in proton-proton interactions at 20, 31, 40, 80 and 158 GeV/c with the NA61/SHINE spectrometer at the CERN SPS

Measurements of inclusive spectra and mean multiplicities of $\pi^\pm$, K$^\pm$, p and $\bar{\textrm{p}}$ produced in inelastic p+p interactions at incident projectile momenta of 20, 31, 40, 80 and 158 GeV/c ($\sqrt{s} = $ 6.3, 7.7, 8.8, 12.3 and 17.3 GeV, respectively) were performed at the CERN Super Proton Synchrotron using the large acceptance NA61/SHINE hadron spectrometer. Spectra are presented as function of rapidity and transverse momentum and are compared to predictions of current models. The measurements serve as the baseline in the NA61/SHINE study of the properties of the onset of deconfinement and search for the critical point of strongly interacting matter.

==> Makefile <==
# Makefile for generating presentation tex related files
# $Id: Makefile 3154 2013-09-26 15:17:51Z darko $

USEPDFLATEX := 1
USEBIBTEX := 1

TARGET := na61Preprint
DEPENDENCIES := $(wildcard plots/* *.tex *.bib include/*bib)

##########################################################

LATEX := $(if $(filter 1, $(USEPDFLATEX)), pdflatex, latex)

COLORIZE := awk 'BEGIN{red="\033[31;1m";yel="\033[34m";byel="\033[34;1m";end="\033[0m"}/Rerun /||/rerunfilecheck[^.]/{e=e$$0"\n";print red""$$0""end;next}/^LaTeX Warning:/||/natbib Warning:/{w=w$$0"\n";print yel""$$0""end;next}{print}END{if(w||e)print "\n"red"Warning/error summary:\n"byel""w""end;if(e)print red""e""end;exit !!e}'

define basic_latex_rule
  for i in 1 2 3 ; do $(LATEX) $< | $(COLORIZE) && exit 0 ; done ; exit 1
endef

ifeq ($(USEBIBTEX), 1)
define latex_rule
  $(LATEX) $<
  bibtex $*
  $(call basic_latex_rule)
endef
else
define latex_rule
  $(call basic_latex_rule)
endef
endif

.PHONY: all clean

all: $(TARGET).pdf

# dependencies
$(TARGET).pdf: $(DEPENDENCIES)

clean:
	- for e in .tex~ .ps .pdf .dvi .log .toc .nav .out .snm .bbl .blg .spl .lof Notes.bib .maf .fff .lot .ttt ; do rm -f $(TARGET)$$e ; done
	- rm -f *.aux include/*.aux

# general rules
ifeq ($(USEPDFLATEX), 1)
%.pdf %.dvi: %.tex $(DEPENDENCIES)
	$(call latex_rule)

%.ps: %.pdf
	pdf2ps $<
else
%.dvi: %.tex $(DEPENDENCIES)
	$(call latex_rule)

%.pdf: %.ps
	ps2pdf $<

%.ps: %.dvi
	dvips $< -o
endif

# embed pdf fonts
%.embedded_fonts.pdf: %.pdf
	gs -dSAFER -dNOPLATFONTS -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sPAPERSIZE=a4 -dCompatibilityLevel=1.4 -dPDFSETTINGS=/printer -dCompatibilityLevel=1.4 -dMaxSubsetPct=100 -dSubsetFonts=true -dEmbedAllFonts=true -sOutputFile=$@ -f $<


==> authors-list.tex <==
\institute{
{National Nuclear Research Center, Baku, Azerbaijan}\label{inst0}
\and{Faculty of Physics, University of Sofia, Sofia, Bulgaria}\label{inst1}
\and{Ru{\dj}er Bo\v{s}kovi\'c Institute, Zagreb, Croatia}\label{inst2}
\and{LPNHE, University of Paris VI and VII, Paris, France}\label{inst3}
\and{Karlsruhe Institute of Technology, Karlsruhe, Germany}\label{inst4}
\and{Fachhochschule Frankfurt, Frankfurt, Germany}\label{inst5}
\and{University of Frankfurt, Frankfurt, Germany}\label{inst6}
\and{University of Athens, Athens, Greece}\label{inst7}
\and{Wigner Research Centre for Physics of the Hungarian Academy of Sciences, Budapest, Hungary}\label{inst8}
\and{Institute for Particle and Nuclear Studies, Tsukuba, Japan}\label{inst9}
\and{University of Bergen, Bergen, Norway}\label{inst10}
\and{Jan Kochanowski University in Kielce, Poland}\label{inst11}
\and{H. Niewodnicza\'nski Institute of Nuclear Physics of the
      Polish Academy of Sciences, Krak\'ow, Poland}\label{inst12}
\and{National Centre for Nuclear Research, Warsaw, Poland}\label{inst13}
\and{Jagiellonian University, Cracow, Poland}\label{inst14}
\and{University of Science and Technology, Cracow, Poland}\label{inst15}
\and{University of Silesia, Katowice, Poland}\label{inst16}
\and{University of Warsaw, Warsaw, Poland}\label{inst17}
\and{University of Wroc{\l}aw,  Wroc{\l}aw, Poland}\label{inst18}
\and{Warsaw University of Technology, Warsaw, Poland}\label{inst19}
\and{Institute for Nuclear Research, Moscow, Russia}\label{inst20}
\and{Joint Institute for Nuclear Research, Dubna, Russia}\label{inst21}
\and{National Research Nuclear University (Moscow Engineering Physics Institute), Moscow, Russia}\label{inst22}
\and{St. Petersburg State University, St. Petersburg, Russia}\label{inst23}
\and{University of Belgrade, Belgrade, Serbia}\label{inst24}
\and{ETH Z\"urich, Z\"urich, Switzerland}\label{inst25}
\and{University of Bern, Bern, Switzerland}\label{inst26}
\and{University of Geneva, Geneva, Switzerland}\label{inst27}
\and{Fermilab, Batavia, USA}\label{inst28}
\and{Los Alamos National Laboratory, Los Alamos, USA}\label{inst29}
\and{University of Colorado, Boulder, USA}\label{inst30}
\and{University of Pittsburgh, Pittsburgh, USA}\label{inst31}
}
\author{
{A.~Aduszkiewicz}\thanksref{inst17}
\and{Y.~Ali}\thanksref{inst14}
\and{E.~Andronov}\thanksref{inst23}
\and{T.~Anti\'ci\'c}\thanksref{inst2}
\and{N.~Antoniou}\thanksref{inst7}
\and{B.~Baatar}\thanksref{inst21}
\and{M.~Baszczyk}\thanksref{inst15}
\and{F.~Bay}\thanksref{inst25}
\and{A.~Blondel}\thanksref{inst27}
\and{M.~Bogomilov}\thanksref{inst1}
\and{A.~Brandin}\thanksref{inst22}
\and{A.~Bravar}\thanksref{inst27}
\and{J.~Brzychczyk}\thanksref{inst14}
\and{S.A.~Bunyatov}\thanksref{inst21}
\and{O.~Busygina}\thanksref{inst20}
\and{P.~Christakoglou}\thanksref{inst7}
\and{M.~\'Cirkovi\'c}\thanksref{inst24}
\and{T.~Czopowicz}\thanksref{inst19}
\and{A.~Damyanova}\thanksref{inst27}
\and{N.~Davis}\thanksref{inst12}
\and{H.~Dembinski}\thanksref{inst4}
\and{M.~Deveaux}\thanksref{inst6}
\and{F.~Diakonos}\thanksref{inst7}
\and{S.~Di~Luise}\thanksref{inst25}
\and{W.~Dominik}\thanksref{inst17}
\and{P.~Dorosz}\thanksref{inst15}
\and{J.~Dumarchez}\thanksref{inst3}
\and{R.~Engel}\thanksref{inst4}
\and{A.~Ereditato}\thanksref{inst26}
\and{G.A.~Feofilov}\thanksref{inst23}
\and{Z.~Fodor}\thanksref{inst8, inst18}
\and{A.~Garibov}\thanksref{inst0}
\and{M.~Ga\'zdzicki}\thanksref{inst6, inst11}
\and{M.~Golubeva}\thanksref{inst20}
\and{K.~Grebieszkow}\thanksref{inst19}
\and{A.~Grzeszczuk}\thanksref{inst16}
\and{F.~Guber}\thanksref{inst20}
\and{A.~Haesler}\thanksref{inst27}
\and{T.~Hasegawa}\thanksref{inst9}
\and{A.E.~Herv\'e}\thanksref{inst4}
\and{M.~Hierholzer}\thanksref{inst26}
\and{J.~Hylen}\thanksref{inst28}
\and{S.~Igolkin}\thanksref{inst23}
\and{A.~Ivashkin}\thanksref{inst20}
\and{S.R.~Johnson}\thanksref{inst30}
\and{K.~Kadija}\thanksref{inst2}
\and{A.~Kapoyannis}\thanksref{inst7}
\and{E.~Kaptur}\thanksref{inst16}
\and{M.~Kie{\l}bowicz}\thanksref{inst12}
\and{J.~Kisiel}\thanksref{inst16}
\and{N.~Knezevi\'c}\thanksref{inst24}
\and{T.~Kobayashi}\thanksref{inst9}
\and{V.I.~Kolesnikov}\thanksref{inst21}
\and{D.~Kolev}\thanksref{inst1}
\and{V.P.~Kondratiev}\thanksref{inst23}
\and{A.~Korzenev}\thanksref{inst27}
\and{~V.~Kovalenko}\thanksref{inst23}
\and{K.~Kowalik}\thanksref{inst13}
\and{S.~Kowalski}\thanksref{inst16}
\and{M.~Koziel}\thanksref{inst6}
\and{A.~Krasnoperov}\thanksref{inst21}
\and{W.~Kucewicz}\thanksref{inst15}
\and{M.~Kuich}\thanksref{inst17}
\and{A.~Kurepin}\thanksref{inst20}
\and{D.~Larsen}\thanksref{inst14}
\and{A.~L\'aszl\'o}\thanksref{inst8}
\and{M.~Lewicki}\thanksref{inst18}
\and{B.~Lundberg}\thanksref{inst28}
\and{V.V.~Lyubushkin}\thanksref{inst21}
\and{M.~Ma\'ckowiak-Paw{\l}owska}\thanksref{inst19}
\and{B.~Maksiak}\thanksref{inst19}
\and{A.I.~Malakhov}\thanksref{inst21}
\and{D.~Mani\'c}\thanksref{inst24}
\and{A.~Marchionni}\thanksref{inst28}
\and{A.~Marcinek}\thanksref{inst14, inst18}
\and{A.D.~Marino}\thanksref{inst30}
\and{K.~Marton}\thanksref{inst8}
\and{H.-J.~Mathes}\thanksref{inst4}
\and{T.~Matulewicz}\thanksref{inst17}
\and{V.~Matveev}\thanksref{inst21}
\and{G.L.~Melkumov}\thanksref{inst21}
\and{~A.~Merzlaya}\thanksref{inst23}
\and{B.~Messerly}\thanksref{inst31}
\and{{\L}.~Mik}\thanksref{inst15}
\and{G.B.~Mills}\thanksref{inst29}
\and{S.~Morozov}\thanksref{inst20, inst22}
\and{S.~Mr\'owczy\'nski}\thanksref{inst11}
\and{Y.~Nagai}\thanksref{inst30}
\and{T.~Nakadaira}\thanksref{inst9}
\and{M.~Naskr\k{e}t}\thanksref{inst18}
\and{M.~Nirkko}\thanksref{inst26}
\and{K.~Nishikawa}\thanksref{inst9}
\and{V.~Ozvenchuk}\thanksref{inst12}
\and{A.D.~Panagiotou}\thanksref{inst7}
\and{V.~Paolone}\thanksref{inst31}
\and{M.~Pavin}\thanksref{inst3, inst2}
\and{O.~Petukhov}\thanksref{inst20, inst22}
\and{C.~Pistillo}\thanksref{inst26}
\and{R.~P{\l}aneta}\thanksref{inst14}
\and{B.A.~Popov}\thanksref{inst21, inst3}
\and{M.~Posiada{\l}a}\thanksref{inst17}
\and{S.~Pu{\l}awski}\thanksref{inst16}
\and{J.~Puzovi\'c}\thanksref{inst24}
\and{R.~Rameika}\thanksref{inst28}
\and{W.~Rauch}\thanksref{inst5}
\and{M.~Ravonel}\thanksref{inst27}
\and{A.~Redij}\thanksref{inst26}
\and{R.~Renfordt}\thanksref{inst6}
\and{E.~Richter-W\k{a}s}\thanksref{inst14}
\and{A.~Robert}\thanksref{inst3}
\and{D.~R\"ohrich}\thanksref{inst10}
\and{E.~Rondio}\thanksref{inst13}
\and{M.~Roth}\thanksref{inst4}
\and{A.~Rubbia}\thanksref{inst25}
\and{B.T.~Rumberger}\thanksref{inst30}
\and{A.~Rustamov}\thanksref{inst0, inst6}
\and{M.~Rybczynski}\thanksref{inst11}
\and{A.~Rybicki}\thanksref{inst12}
\and{A.~Sadovsky}\thanksref{inst20}
\and{K.~Sakashita}\thanksref{inst9}
\and{R.~Sarnecki}\thanksref{inst19}
\and{K.~Schmidt}\thanksref{inst16}
\and{T.~Sekiguchi}\thanksref{inst9}
\and{I.~Selyuzhenkov}\thanksref{inst22}
\and{A.~Seryakov}\thanksref{inst23}
\and{P.~Seyboth}\thanksref{inst11}
\and{D.~Sgalaberna}\thanksref{inst25}
\and{M.~Shibata}\thanksref{inst9}
\and{M.~S{\l}odkowski}\thanksref{inst19}
\and{P.~Staszel}\thanksref{inst14}
\and{G.~Stefanek}\thanksref{inst11}
\and{J.~Stepaniak}\thanksref{inst13}
\and{H.~Str\"obele}\thanksref{inst6}
\and{T.~\v{S}u\v{s}a}\thanksref{inst2}
\and{M.~Szuba}\thanksref{inst4}
\and{M.~Tada}\thanksref{inst9}
\and{A.~Taranenko}\thanksref{inst22}
\and{A.~Tefelska}\thanksref{inst19}
\and{D.~Tefelski}\thanksref{inst19}
\and{V.~Tereshchenko}\thanksref{inst21}
\and{R.~Tsenov}\thanksref{inst1}
\and{L.~Turko}\thanksref{inst18}
\and{R.~Ulrich}\thanksref{inst4}
\and{M.~Unger}\thanksref{inst4}
\and{M.~Vassiliou}\thanksref{inst7}
\and{D.~Veberi\v{c}}\thanksref{inst4}
\and{V.V.~Vechernin}\thanksref{inst23}
\and{G.~Vesztergombi}\thanksref{inst8}
\and{L.~Vinogradov}\thanksref{inst23}
\and{~M.~Walewski}\thanksref{inst17}
\and{A.~Wickremasinghe}\thanksref{inst31}
\and{A.~Wilczek}\thanksref{inst16}
\and{Z.~W{\l}odarczyk}\thanksref{inst11}
\and{A.~Wojtaszek-Szwarc}\thanksref{inst11}
\and{O.~Wyszy\'nski}\thanksref{inst14}
\and{L.~Zambelli}\thanksref{inst3, inst9}
\and{E.D.~Zimmerman}\thanksref{inst30}
\and{R.~Zwaska}\thanksref{inst28}
}


==> sections/00-abstract.tex <==
\begin{abstract}
Measurements of inclusive spectra and mean multiplicities of $\pi^\pm$, K$^\pm$, p and $\bar{\text{p}}$ produced in inelastic p+p interactions at incident projectile momenta of 20, 31, 40, 80 and 158~\GeVc ($\sqrt{s} = $ 6.3, 7.7, 8.8, 12.3 and 17.3~\GeV, respectively) were performed at the CERN Super Proton Synchrotron using the large acceptance \NASixtyOne hadron spectrometer. Spectra are presented as function of rapidity and transverse momentum. The measurements are part of the \NASixtyOne programme on strong interactions devoted to the study of the properties of the onset of deconfinement and search for the critical point of strongly interacting matter as the detailed knowledge of basic interaction is essential for the extraction of hot matter effects. 
%They are required for interpretation of results on nucleus-nucleus and proton-nucleus collisions.
\end{abstract}


==> sections/02-dataprocess.tex <==
\section{Data processing and simulation}\label{sec:dataprocess}

Detector parameters were optimized by a data-based calibration procedure which also took into account their time dependence. Small adjustments were determined in consecutive steps for:
\begin{enumerate}
  \item detector geometry, drift velocities in TPCs and distortions due to the inhomogeneities of the magnetic field in the corners of the VTPC detectors,
  \item magnetic field settings,
  \item specific energy loss measurements,
  \item time-of-flight measurements.
\end{enumerate}
Each step required reconstruction of the data in order to optimize a set of calibration constants and time dependent corrections followed by verification procedures. 

Data reconstruction was performed accordingly to the following steps:
\begin{enumerate}
  \item extraction of the cluster in the TPC raw data, calculation of its center-of-gravity and total charge,
  \item reconstruction of track segments sections in each TPC separately,
  \item matching track segments into global TPCs tracks,
  \item fitting track through the magnetic field and determination of its parameters at the first measured TPC cluster,
  \item determination of the interaction vertex using the beam trajectory ($x$ and $y$ coordinates) fitted in the BPDs and the trajectories of tracks reconstructed in the TPCs ($z$ coordinate),
  \item refitting the particle trajectory using the interaction vertex as an additional point and determination of the particle momentum at the interaction vertex,
  \item matching of ToF hits with the TPC tracks.
\end{enumerate}


A simulation of the \NASixtyOne detector response is used to correct the reconstructed data. Several Monte-Carlo (MC) models predictions were compared with the \NASixtyOne experimental results on p+p, p+C and $\pi$+C interactions: FLUKA 2008~\cite{Ferrari:2005zk,Bohlen2014211}, URQMD 1.3.1~\cite{Bass:1998ca,Bleicher:1999xi}, VENUS 4.12~\cite{Werner:1993uh}, EPOS 1.99~\cite{Werner:2008zza}, GHEISHA 2002~\cite{Mishev:2014wka}, QGSJetII-3~\cite{Pierog:2007zza} and Sibyll~2.1~\cite{Ahn:2009wx,M.Ungerforthe:2013aha,Unger:2010ze}. Based on these comparisons and taking into account continuous support and documentation from the developers the EPOS model was selected. 

The simulation consists of the following steps:
\begin{enumerate}
  \item generation of inelastic interactions,
  \item propagation of outgoing particles through the detector material using the GEANT 3.21 package~\cite{Geant3}, taking into account the magnetic field and relevant physics processes, such as particle interactions and decays,
  \item simulation of the detector response using dedicated \NASixtyOne packages which introduce distortions corresponding to all corrections applied to the physical data,
  \item storage of the simulated events in a file which has the same format as the raw data,
  \item reconstruction of the simulated events with the reconstruction chain used for the reconstruction of experimental data,
  \item matching of the reconstructed tracks to the simulated ones based on the cluster positions.
\end{enumerate}

Only inelastic p+p interactions in the hydrogen in the target cell were simulated and reconstructed. Therefore, the corrections based on Monte Carlo can be applied only for inelastic events. The contribution of elastic events is eliminated by the event selection cuts, whereas the contribution of off-target interactions is subtracted by specially collected events with empty LHT.



==> sections/06-finalcalculations.tex <==
\section{Corrected spectra and uncertainties}\label{sec:results_calc}

%---------------------------------------------------------------------------------------

	\subsection{Final multiplicities calculations and statistical uncertainties}
		
		Multiplicity of different hadrons from inelastic p+p interactions measured by the \dedx technique is defined as a sum of probabilities divided by the number of events corrected for detector effects, feed-down and out of target contamination. For particle type $i=\pi^{-},\ \pi^{+},\ K^{-},\ K^{+},\ \bar{p},\ p$, it is defined as:
		\begin{equation}
		\label{finalresdEdx}
		\frac{n_{i}}{N}=
		\frac{1}{C}
		\frac{\sum\limits_{I} P_{i}(p_{tot},p_{T},dE/dx) - B \sum\limits_{R} P_{i}(p_{tot},p_{T},dE/dx)}{N_{I} - B N_{R}},
		\end{equation}
		
		where:
		\begin{itemize}
		\item $C$ - correction factor defined in Eq.~\ref{eq:corectionfactor},
		\item $\sum\limits_{I} P_{i}(p_{tot},p_{T},dE/dx) \equiv \sum\limits_{I} P_{i}$ - sum over probabilities $P_{i}$ defined in Eq.~\ref{eq:propdedx} of all tracks for inserted target (abbreviated as "I"), 
		\item $\sum\limits_{R} P_{i}(p_{tot},p_{T},dE/dx) \equiv \sum\limits_{R} P_{i}$ - sum over probabilities $P_{i}$ defined in Eq.~\ref{eq:propdedx} for all tracks for removed target (abbreviated as "R"),
		\item $B$ - the normalization factor (see Chapter~\ref{outtarget}),
		\item $N_{I}$ and $N_{R}$ - the number of events of target inserted and removed, respectively.
		\end{itemize}

Statistical error of multiplicities obtained by \dedx method has been calculated in the following way:
\begin{equation}
\begin{split}
	\left(\Delta\frac{n_{i}}{N}\right)^{2} =
	\left(\left|\frac{-1}{C^{2}} \frac{\sum\limits_{I} P_{i} - B \sum\limits_{R} P_{i}}{N_{I} - B N_{R}}\right| \Delta C \right)^{2} + \\
	\left(\left|\frac{1}{C} \frac{1}{N_{I} - B N_{R}}\right| \sqrt{\sum\limits_{I}P_{i}}\right)^{2} + \\ 
	\left(\left|\frac{1}{C} \frac{-B}{N_{I} - B N_{R}}\right| \sqrt{\sum\limits_{R}P_{i}}\right)^{2}  \ ,
\end{split} 
\end{equation}
where: $\Delta$ devote statistical uncertainty of the variables used to calculate particle multiplicity. Uncertainty of normalization factor ($B$) as well as number of events ($N_{I}$ and $N_{R}$) are not taken into account during this calculation due to their negligible influence on the uncertainty value.

%Example of obtained by \dedx identification and corrected spectra in p+p interactions at $40~GeV/c$ is presented in Fig.~\ref{fig:dedxmult}
%
%\begin{figure}[!ht]
%	\begin{center}
%	\includegraphics[width=0.15\textwidth]{ch8/ded_npi}
%	\includegraphics[width=0.15\textwidth]{ch8/ded_nka}
%	\includegraphics[width=0.15\textwidth]{ch8/ded_npr}\\
%	\includegraphics[width=0.15\textwidth]{ch8/ded_ppi}
%	\includegraphics[width=0.15\textwidth]{ch8/ded_pka}
%	\includegraphics[width=0.15\textwidth]{ch8/ded_ppr}
%	\end{center}
%	\caption{(Color online) Multiplicity of $\pi^+$, $\pi^{-}$, $K^{+}$, $K^{-}$, $p$ and $\bar{p}$ from p+p inelastic interactions at $40~GeV/c$ from \dedx method.}
%	\label{fig:dedxmult}
%\end{figure}

Particle multiplicities for $tof$-\dedx technique can be calculated in a similar way (exception are corrections factors). In this case, particle yields are defined as:
		\begin{equation}
		\label{finalrestof}
		\frac{n_{i}}{N}=
		\frac{1}{C_{tof}}
		\frac{\sum\limits_{I} \frac{P_{i}(p_{tot},p_{T},dE/dx,tof)}{\epsilon} - B \sum\limits_{R} \frac{P_{i}(p_{tot},p_{T},dE/dx,tof)}{\epsilon}}{N_{I} - B N_{R}} ,
		\end{equation}
where: $P_{i}$ are the probabilities defined in Eq.~\ref{eq:proptof}, $\epsilon$ - efficiency described by Eq.~\ref{eq:correctiontof} and $C_{tof}$ - the correction for the losses due to the momentum acceptance of the fitting procedure. 

	Statistical error estimation of the multiplicities calculated by the $tof$-\dedx technique is more complicated. It was assumed that $\epsilon$ statistical error is equal to the mean statistical uncertainty in full $y-p_{T}$ bin, and therefore it can be moved in front of the sums. Finally, statistical error can be calculated according to the following formula
	\begin{equation}
	\begin{split}
	\left(\Delta\frac{n_{i}}{N}\right)^{2} = 	\left(\left|\frac{-1}{C_{tof}^{2}} \frac{\sum\limits_{I} \frac{P_{i}}{\epsilon} - B \sum\limits_{R} \frac{P_{i}}{\epsilon}}{N_{I} - B N_{R}}\right| \Delta C_{tof} \right)^{2} + \\
	\left(\left|\frac{1}{C_{tof}} \frac{\sum\limits_{I}\frac{1}{\epsilon}}{N_{I} - B N_{R}}\right| \sqrt{\sum\limits_{I}P_{i}}\right)^{2} + \\ 
	\left(\left|\frac{1}{C_{tof}} \frac{\sum\limits_{R}\frac{-B}{\epsilon}}{N_{I} - B N_{R}}\right| \sqrt{\sum\limits_{R}P_{i}}\right)^{2} + \\
	\left(\left|\frac{-1}{C_{tof} \langle \epsilon \rangle^2} \frac{\sum\limits_{I} P_{i} - B \sum\limits_{R} P_{i}}{N_{I} - B N_{R}}\right| \langle \Delta \epsilon \rangle\ \right)^{2} .
\end{split} 
	\end{equation}
	
%	Spectra of $\pi^+$, $\pi^{-}$, $K^{+}$, $K^{-}$ and $p$ produced in inelastic p+p at $40~GeV/c$ obtained by $tof-dEdx$ method are shown in Fig.~\ref{fig:tofmult}.

%\begin{figure}[!ht]
%	\begin{center}
%	\includegraphics[width=0.15\textwidth]{ch8/tof_npi}
%	\includegraphics[width=0.15\textwidth]{ch8/tof_nka}\\
%	\includegraphics[width=0.15\textwidth]{ch8/tof_ppi}
%	\includegraphics[width=0.15\textwidth]{ch8/tof_pka}
%	\includegraphics[width=0.15\textwidth]{ch8/tof_ppr}
%	\end{center}
%	\caption{(Color online) Multiplicity of $\pi^+$, $\pi^{-}$, $K^{+}$, $K^{-}$ and $p$ from p+p inelastic interactions at $158~GeV/c$ from $tof$-\dedx method.}
%	\label{fig:tofmult}
%\end{figure}
	
	\subsection{Systematic uncertainty of measured multiplicities}
	
	The main systematic biases to the measurement could come from:
	\begin{itemize}
	\item event and track cuts which are not corrected,
	\item event losses due to trigger settings,
	\item methods of track and event selection,
	\item used identification techniques.
	\end{itemize}

	The first possible uncertainty is related to the event and track cuts for which are not corrected for. The main source of such bias can be assign to the off-time particles. Therefore, to estimate this systematic uncertainty, selections criteria has been changed. The analysis was performed with different time windows in which second beam particle can be observed in the same event (WFA $\pm~1~\mu s$ over nominal one). This results were compared with the nominal one and maximum difference between them was assign as the systematic uncertainty of the measurement.
	
	Second source of the systematic bias are the event losses connected to the trigger settings. During the data taking, in the trigger system, the S4 detector was used to remove from the data elastic events. However, such configuration can also result in losses of the inelastic events. To take into account this effect, identification procedure has to be done with Monte-Carlo correction calculated with and without S4 counter. Difference between this two results allow to estimate this systematic error.
	
	The next source of the systematic bias are track and event selection methods. To calculate the effect of the selection criteria for the results, following variations of them were performed independently:
	\begin{itemize}
	\item number of requested points of track in all TPCs was changed by $\pm$5,
	\item number of requested points of track in VTPCs was reduced or enlarge by 5,
	\item position of fitted vertex was checked in the range of $\pm$10\cm around the nominal value.
	\end{itemize}
	
	Moreover, additional biases of the \dedx method have been studied and estimated by the 10\% variation of the parameter limits for function used for particle identification. In case of $tof$-\dedx identification source of the possible uncertainty were found by changing the selection criteria related to this technique. The systematic uncertainties for the \dedx method, for selected $p_{T}$ interval and beam momentum of 40\GeV/c are presented in Fig.~\ref{fig:sysexa}.
	
	\begin{figure}[!ht]
		\begin{center}
		\includegraphics[width=0.8\textwidth]{ch8/sys}
		\end{center}
		\caption{(Color online)\textcolor{red}{Plot to be exchanged and additional one from tof}
 Systematic uncertainty components in p+p interaction at $40~GeV/c$ as the function of rapidity for transverse momentum interval between $0.3$ and $0.4~GeV/c$.}
		\label{fig:sysexa}
	\end{figure}
	
	Assuming the independence of all systematic error sources, the final systematic uncertainty has been calculated as a square root of sum squares of the above described components.
	
	\textcolor{red}{Comparisons with world data}
Production of positive and negative pions, kaons and protons in p+p interactions at 158\GeVc was measured only by the NA49 experiment~\cite{Anticic:2010yg,Alt:2005zq,Anticic:2009wd}. Comparison of \NASixtyOne and NA49 rapidity distributions is presented in Fig~\ref{fig:withna49}. 

\begin{figure}[!ht]
	\begin{center}
	\includegraphics[width=0.3\textwidth]{ch9/comp/fischerpim}
	\includegraphics[width=0.3\textwidth]{ch9/comp/fischerpip}\\
	\includegraphics[width=0.3\textwidth]{ch9/comp/fischerkm}
	\includegraphics[width=0.3\textwidth]{ch9/comp/fischerkp}\\
	\includegraphics[width=0.3\textwidth]{ch9/comp/fischerap}
	\includegraphics[width=0.3\textwidth]{ch9/comp/fischerp}
	\end{center}
	\caption{(Color online)\textcolor{red}{Plot to be exchanged} Comparison of rapidity distributions of pions, kaons and protons produced in p+p interactions at 158\GeVc. The NA49 results were published without quotation of uncertainties.}
	\label{fig:withna49}
\end{figure}

The \NASixtyOne experiment published also $\pi^{-}$ spectra at all presented energies obtained by method so-called $h^{-}$~\cite{Abgrall:2013qoa}. This technique is based on the fact that the majority of negatively charged particles are $\pi^{-}$ mesons. Contribution of the other particles is subtracted using \Epos model. Comparison of $h^{-}$ method results with the results presented in this publication is shown in Fig~\ref{fig:withantoni}. All methods give results which are in agreement within uncertainties.

\begin{figure}[!ht]
	\begin{center}
	\includegraphics[width=0.3\textwidth]{ch9/comp/a20}
	\includegraphics[width=0.3\textwidth]{ch9/comp/a30}\\
	\includegraphics[width=0.3\textwidth]{ch9/comp/a40}
	\includegraphics[width=0.3\textwidth]{ch9/comp/a80}\\
	\includegraphics[width=0.3\textwidth]{ch9/comp/a158}
	\includegraphics[width=0.3\textwidth]{ch9/comp/legend}
	\end{center}
	\caption{(Color online)\textcolor{red}{Plot to be exchanged and check of 40 GeV plot.}  Comparison of $\pi^{-}$ rapidity distribution obtained by \dedx and $tof$-\dedx methods with $h^{-}$ technique.}
	\label{fig:withantoni}
\end{figure}

==> sections/07-results.tex <==
\section{Results}
\label{sec:results}

	\subsection{Particle production in $y$ vs $p_{T}$ phase space}
	Two dimensional spectra ($y$ vs. $p_{T}$) of $\pi^{-}$, $\pi^{+}$, $K^{-}$, $K^{+}$, $p$ and $\bar{p}$ produced in inelastic p+p interactions at different SPS energies are presented in Fig~\ref{fig:final2D}. The anti-protons at 20\GeVc were not identified due to limited statistics of collected data. It can be noticed that, the particles production increases with collision energy. That behaviour is observed for all particles types. Empty bins in the phase-space (mostly for lower energies) are caused by missing acceptance of the methods used for analysis.
	
\begin{figure*}
\begin{center}
\newcolumntype{S}{>{\centering} m{0.03\textwidth} }
\newcolumntype{A}{>{\centering} m{0.13\textwidth} }
%\begin{table}[!ht]
\hspace{-10mm}
\begin{tabular}{S A A A A A A}%c@{}c@{}c@{}c@{}c}
%& $\pi^{-}$ & $\pi^{+}$ & $K^{-}$ & p 
& \tiny20\GeVc & \tiny31\GeVc & \tiny40\GeVc & \tiny80\GeVc  & \tiny158\GeVc 
\tabularnewline
%\begin{sideways} $\pi^{-}$ \end{sideways} &
\vspace{-5mm}$\pi^{-}$ &
\includegraphics[width=0.12\textwidth]{ch9/pim20} &
\includegraphics[width=0.12\textwidth]{ch9/pim30} &
\includegraphics[width=0.12\textwidth]{ch9/pim40} &
\includegraphics[width=0.12\textwidth]{ch9/pim80} &
\includegraphics[width=0.12\textwidth]{ch9/pim158} 
\tabularnewline
\vspace{-5mm}$\pi^{+}$ &
\includegraphics[width=0.12\textwidth]{ch9/pip20} &
\includegraphics[width=0.065\textwidth]{ch9/pip30} &
\includegraphics[width=0.12\textwidth]{ch9/pip40} &
\includegraphics[width=0.12\textwidth]{ch9/pip80} &
\includegraphics[width=0.12\textwidth]{ch9/pip158} 
\tabularnewline
\vspace{-5mm}$K^{-}$ &
\includegraphics[width=0.12\textwidth]{ch9/Km20} &
\includegraphics[width=0.12\textwidth]{ch9/Km30} &
\includegraphics[width=0.12\textwidth]{ch9/Km40} &
\includegraphics[width=0.12\textwidth]{ch9/Km80} &
\includegraphics[width=0.12\textwidth]{ch9/Km158} 
\tabularnewline
\vspace{-5mm}$K^{+}$ &
\includegraphics[width=0.12\textwidth]{ch9/Kp20} &
\includegraphics[width=0.12\textwidth]{ch9/Kp30} &
\includegraphics[width=0.12\textwidth]{ch9/Kp40} &
\includegraphics[width=0.12\textwidth]{ch9/Kp80} &
\includegraphics[width=0.12\textwidth]{ch9/Kp158} 
\tabularnewline
\vspace{-5mm}$p$ &
\includegraphics[width=0.12\textwidth]{ch9/p20} &
\includegraphics[width=0.12\textwidth]{ch9/p30} &
\includegraphics[width=0.12\textwidth]{ch9/p40} &
\includegraphics[width=0.12\textwidth]{ch9/p80} &
\includegraphics[width=0.12\textwidth]{ch9/p158} 
\tabularnewline
\vspace{-5mm}$\bar{p}$ &
&
\includegraphics[width=0.12\textwidth]{ch9/ap30} &
\includegraphics[width=0.12\textwidth]{ch9/ap40} &
\includegraphics[width=0.12\textwidth]{ch9/ap80} &
\includegraphics[width=0.12\textwidth]{ch9/ap158} 
\tabularnewline
\end{tabular}
%\end{table}
		%\includegraphics[width=0.9\textwidth]{}
		\end{center}
		\caption{(Color online) Two dimensional spectra of $\pi^{-}$, $\pi^{+}$, $K^{-}$, $K^{+}$, $p$ and $\bar{p}$ produced in inelastic p+p interactions at 20, 31, 40, 80 and 158\GeVc. Color scale represents particle multiplicities normalized to the phase-space bin size ($\frac{dn}{dydp_{T}}$).}
		\label{fig:final2D}
	\end{figure*}
	
	Multiplicities presented in Fig.~\ref{fig:final2D} can be studied as a function of rapidity ($y$) or transverse momentum ($p_{T}$). Transverse mass distributions of $K^{-}$, $K^{+}$ produced in p+p interactions at 20, 31, 40, 80, 158\GeVc as the function of rapidity are presented in Figs.~\ref{fig:nptkaon} and \ref{fig:pptkaon}, respectively. Additionally, double differential $p_{T}$ spectra of $\pi^{-}$ and $\pi^{+}$ are shown in Figs.~\ref{fig:nptpion}, \ref{fig:pptpion} for five SPS energies. Spectra are scaled by appropriate factors for better separation. Shadow band in the figures correspond to systematic uncertainties of double differential spectra.
	
\begin{figure*}
		\begin{center}
		\includegraphics[width=0.18\textwidth]{ch9/pt/Km20}
		\includegraphics[width=0.18\textwidth]{ch9/pt/Km30}
		\includegraphics[width=0.18\textwidth]{ch9/pt/Km40}
		\includegraphics[width=0.18\textwidth]{ch9/pt/Km80}
		\includegraphics[width=0.18\textwidth]{ch9/pt/Km158}
		\end{center}
		\caption{(Color online) $K^{-}$ spectra produced in inelastic p+p interactions at 20, 31, 40, 80, 158\GeVc beam momentum. Rapidity values on the figure correspond to the middle of the presented bin.}
		\label{fig:nptkaon}
\end{figure*}
	
\begin{figure*}
		\begin{center}
		\includegraphics[width=0.18\textwidth]{ch9/pt/Kp20}
		\includegraphics[width=0.18\textwidth]{ch9/pt/Kp30}
		\includegraphics[width=0.18\textwidth]{ch9/pt/Kp40}
		\includegraphics[width=0.18\textwidth]{ch9/pt/Kp80}
		\includegraphics[width=0.18\textwidth]{ch9/pt/Kp158}
		\end{center}
		\caption{(Color online) $K^{+}$ spectra produced in inelastic p+p interactions at 20, 31, 40, 80, 158\GeVc beam momentum. Rapidity values on the figure correspond to the middle of the presented bin.}
		\label{fig:pptkaon}
\end{figure*}
	
\begin{figure*}
		\begin{center}
		\includegraphics[width=0.18\textwidth]{ch9/pt/pim20}
		\includegraphics[width=0.18\textwidth]{ch9/pt/pim30}
		\includegraphics[width=0.18\textwidth]{ch9/pt/pim40}
		\includegraphics[width=0.18\textwidth]{ch9/pt/pim80}
		\includegraphics[width=0.18\textwidth]{ch9/pt/pim158}
		\end{center}
		\caption{(Color online) $\pi^{-}$ spectra produced in inelastic p+p interactions at 20, 31, 40, 80, 158\GeVc beam momentum. Rapidity values on the figure correspond to the middle of the presented bin.}
		\label{fig:nptpion}
\end{figure*}

\begin{figure*}
		\begin{center}
		\includegraphics[width=0.18\textwidth]{ch9/pt/pip20}
		\includegraphics[width=0.18\textwidth]{ch9/pt/pip30}
		\includegraphics[width=0.18\textwidth]{ch9/pt/pip40}
		\includegraphics[width=0.18\textwidth]{ch9/pt/pip80}
		\includegraphics[width=0.18\textwidth]{ch9/pt/pip158}
		\end{center}
		\caption{(Color online) $\pi^{+}$ spectra produced in inelastic p+p interactions at 20, 31, 40, 80, 158\GeVc beam momentum. Rapidity values on the figure correspond to the middle of the presented bin.}
		\label{fig:pptpion}
\end{figure*}
		
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%		
%%%		\begin{figure}[!ht]
%%%		\begin{center}
%%%		\includegraphics[width=0.22\textwidth]{ch9/pt/pim20}
%%%		\includegraphics[width=0.22\textwidth]{ch9/pt/pip20}
%%%		\end{center}
%%%		\caption{Double differential spectra of positively and negatively charged pions produced in inelastic p+p interactions at 20\GeVc beam momentum. Rapidity values on the figure correspond to the middle of the presented bin.}
%%%		\label{fig:ptpion20}
%%%	\end{figure}
%%%	
%%%	\begin{figure}[!ht]
%%%		\begin{center}
%%%		\includegraphics[width=0.22\textwidth]{ch9/pt/pim30}
%%%		\includegraphics[width=0.22\textwidth]{ch9/pt/pip30}
%%%		\end{center}
%%%		\caption{Double differential spectra of positively and negatively charged pions produced in inelastic p+p interactions at 31\GeVc beam momentum. Rapidity values on the figure correspond to the middle of the presented bin.}
%%%		\label{fig:ptpion30}
%%%	\end{figure}
%%%	
%%%	\begin{figure}[!ht]
%%%		\begin{center}
%%%		\includegraphics[width=0.22\textwidth]{ch9/pt/pim40}
%%%		\includegraphics[width=0.22\textwidth]{ch9/pt/pip40}
%%%		\end{center}
%%%		\caption{Double differential spectra of positively and negatively charged pions produced in inelastic p+p interactions at 40\GeVc beam momentum. Rapidity values on the figure correspond to the middle of the presented bin.}
%%%		\label{fig:ptpion40}
%%%	\end{figure}
%%%	
%%%	\begin{figure}[!ht]
%%%		\begin{center}
%%%		\includegraphics[width=0.22\textwidth]{ch9/pt/pim80}
%%%		\includegraphics[width=0.22\textwidth]{ch9/pt/pip80}
%%%		\end{center}
%%%		\caption{Double differential spectra of positively and negatively charged pions produced in inelastic p+p interactions at 80\GeVc beam momentum. Rapidity values on the figure correspond to the middle of the presented bin.}
%%%		\label{fig:ptpion80}
%%%	\end{figure}
%%%			
%%%	\begin{figure}[!ht]
%%%		\begin{center}
%%%		\includegraphics[width=0.22\textwidth]{ch9/pt/pim158}
%%%		\includegraphics[width=0.22\textwidth]{ch9/pt/pip158}
%%%		\end{center}
%%%		\caption{Double differential spectra of positively and negatively charged pions spectra produced in inelastic p+p interactions at 158\GeVc beam momentum. Rapidity values on the figure correspond to the middle of the presented bin.}
%%%		\label{fig:ptpion158}
%%%	\end{figure}

%%	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	It was mentioned that the particle production can be presented as the function of the transverse momentum. The rapidity distribution of protons and anti-protons produced in inelastic p+p interactions at 31, 40, 80 and 158\GeVc for transverse momentum intervals are shown in Figs.~\ref{fig:ppy}, \ref{fig:appy}. The spectra are symmetrical around the mid-rapidity ($y=0$). 
	
	 \begin{figure*}
	 	\begin{center}
	 	\includegraphics[width=0.22\textwidth]{ch9/pt/p30}
	 	\includegraphics[width=0.22\textwidth]{ch9/pt/p40}
	 	\includegraphics[width=0.22\textwidth]{ch9/pt/p80}
	 	\includegraphics[width=0.22\textwidth]{ch9/pt/p158}
	 	\end{center}
	 	\caption{(Color online)\textcolor{red}{Plots to be exchanged by pt?} Double differential rapidity spectra of protons from p+p at 31, 40, 80 and 158\GeVc for different transverse momentum intervals.}
	 	\label{fig:ppy}
	 \end{figure*}
	 
	 \begin{figure*}
	 	\begin{center}
	 	\includegraphics[width=0.22\textwidth]{ch9/pt/ap30}
	 	\includegraphics[width=0.22\textwidth]{ch9/pt/ap40}
	 	\includegraphics[width=0.22\textwidth]{ch9/pt/ap80}
	 	\includegraphics[width=0.22\textwidth]{ch9/pt/ap158}
	 	\end{center}
	 	\caption{(Color online)\textcolor{red}{Plots to be exchanged by pt?} Double differential rapidity spectra of protons from p+p at 31, 40, 80 and 158\GeVc for different transverse momentum intervals.}
	 	\label{fig:appy}
	 \end{figure*}
	 		

	

==> sections/08-4pi.tex <==
\section{Rapidity distribiutions and mean multiplicities}\label{sec:4pi}		

	Calculation of mean multiplicities have been also performed. Firstly, the extrapolation to not measure phase-space region in $p_T$ by the exponential function fit and then reflection of the result around mid-rapidity ($y=0$) to the backward hemisphere was done. The reflection can be done thanks to the symmetrical collision system. Thus, calculations for the backward rapidity region for some bins of transverse momentum can be performed.
		
	Next, $4\pi$ multiplicities distribution for positive hemisphere of particle production are integrated and extrapolated over transverse momentum. Results of this procedure are presented in Fig.~\ref{fig:finaldndy}. Statistical error, visible as a bars, are calculated as the square root of sum of the squares statistical errors of measured point and exponential fit. The systematic uncertainty (shadow bands) is a square root of sum of the squares measured systematic uncertainty and half of the extrapolated yield. Visible lines corresponds to the fits with sum of two identical Gaussian functions with mean position symmetrically displaced around mid-rapidity. Such function was selected, hence it gives the best description of the data.
	
	\begin{figure}[!ht]
		\begin{center}
		\includegraphics[width=0.4\textwidth]{ch9/kplusdndy}
		\includegraphics[width=0.4\textwidth]{ch9/kminusdndy}\\
		\includegraphics[width=0.4\textwidth]{ch9/piplusdndy}
		\includegraphics[width=0.4\textwidth]{ch9/piminusdndy}\\
		\includegraphics[width=0.4\textwidth]{ch9/protonsdndy}
		\includegraphics[width=0.4\textwidth]{ch9/antiprotonsdndy}
		\end{center}
		\caption{(Color online) Rapidity spectra of different particles at SPS energies range, scaled by appropriate factors for better separation.}
		\label{fig:finaldndy}
	\end{figure}
	
	Study of the proton production in p+p interactions by the NA49 experiment~\cite{Baatar:2012fua} and it's comparison to theoretical model excluded possibility to calculate $4\pi$ proton multiplicity based on the Monte-Carlo models. Comparison of presented \NASixtyOne results, NA49 measurement and theoretical models: \Urqmd~\cite{Bass:1998ca,Bleicher:1999xi}, \Epos~\cite{Werner:2008zza} is presented in Fig.~\ref{fig:protonmodel}. It can be observed that models do not described well high momentum (rapidity) region for protons at 158\GeVc.
	
	\begin{figure}
		\begin{center}
		\includegraphics[width=0.3\textwidth]{ch9/dndyprotons_model}
		\end{center}
		\caption{(Color online) \textcolor{red}{Plot will be removed mean mult calculated base on models...} Proton rapidity distribution at 158\GeVc compered with NA49 measurement and Monte-Carlo models.}
		\label{fig:protonmodel}
	\end{figure}
	
	The multiplicity of $\pi^{+}$, $\pi^{-}$, $K^{+}$, $K^{-}$ and $\bar{p}$ per inelastic event were calculated using results presented in Fig.~\ref{fig:finaldndy}. The mean number of produced particles with the statistical and systematic uncertainties is summarized in Tables~\ref{tab:meanmultp} and~\ref{tab:meanmultn}, for positively and negatively charged particles, respectively.
	
	
	\begin{table}
%	\resizebox{\textwidth}{!}{
	\begin{center}
	\begin{tabular}{ c || c | c }
    & \tiny$K^{+}$ & \tiny$\pi^{+}$ \\
	\hline
	\hline
	\tiny20\GeVc   & \tiny$ 0.097\pm 0.014\pm 0.0062$ & \tiny$ 1.582\pm 0.122\pm 0.197$ \\
	\tiny31\GeVc & \tiny$ 0.157\pm 0.010\pm 0.015$  & \tiny$1.985\pm 0.210\pm 0.197$ \\
	\tiny40\GeVc   & \tiny$ 0.170\pm 0.009\pm 0.023$  & \tiny$ 2.221\pm 0.220\pm 0.164$ \\
	\tiny80\GeVc   & \tiny$ 0.201\pm 0.010\pm 0.010$  & \tiny$ 2.556\pm 0.220\pm 0.140$ \\
	\tiny158\GeVc  & \tiny$ 0.234\pm 0.014\pm 0.017$  & \tiny$ 2.991\pm 0.305\pm 0.250$ \\
	\hline
	\end{tabular}
	\end{center}
%	}
	\caption{Mean multiplicity of positive particles at SPS energies with statistical and systematic uncertainties.}
	\label{tab:meanmultp}
	\end{table}	

	\begin{table}
%	\end{table}
%	\resizebox{\textwidth}{!}{
	\begin{center}
	\begin{tabular}{ c || c | c | c}
    & \tiny$K^{-}$ & \tiny$\pi^{-}$& \tiny$\bar{p}$\\
	\hline
	\hline
	\tiny20\GeVc   & \tiny$ 0.024\pm 0.006\pm 0.002$ & \tiny$ 1.067\pm 0.053\pm 0.196$ &\tiny  --- \\
	\tiny31\GeVc & \tiny$ 0.045\pm 0.004\pm 0.003$ &\tiny $ 1.438\pm 0.219\pm 0.187$ &\tiny $ 0.0047\pm 0.0007\pm 0.0003$  \\
	\tiny40\GeVc   & \tiny$ 0.084\pm 0.006\pm 0.003$ &\tiny $ 1.703\pm 0.192\pm 0.213$ &\tiny $ 0.0059\pm 0.0006\pm 0.0004$  \\
	\tiny80\GeVc   & \tiny$ 0.095\pm 0.004\pm 0.005$ &\tiny $ 2.030\pm 0.248\pm 0.132$ &\tiny $ 0.0183\pm 0.0015\pm 0.0011$  \\
	\tiny158\GeVc  & \tiny$ 0.132\pm 0.011\pm 0.009$ &\tiny $ 2.494\pm 0.259\pm 0.179$ &\tiny $ 0.0402\pm 0.0020\pm 0.0026$  \\
	\hline
	\end{tabular}
	\end{center}
%	}
	\caption{Mean multiplicity of negative particles at SPS energies with statistical and systematic uncertainties.}
	\label{tab:meanmultn}
	\end{table}

\subsection{Energy dependence of mean particle production in p+p interactions}

Investigation of p+p interactions for mean multiplicity of positive and negative kaons exhibit different trends. It increases with the collision energy ($\sqrt{S_{NN}}$). This dependence is presented in Fig.~\ref{fig:Kaonmeanmult}. The \NASixtyOne results are presented together with the existing world data~\cite{Anticic:2010yg,Gazdzicki:1996pk,Gazdzicki:1991ih,Bachler:1999hu,Verbeure:1991tv,Rossi:1974if,Golokhvastov:2001ei,Becattini:1997rv,Back:2003xk}. The most of the world data points came from bubble chambers experiments and they are presented without the error bars (statistical uncertainty of $20-70\%$). 

\begin{figure}[!ht]
	\begin{center}
	\includegraphics[width=0.46\textwidth]{ch10/meankp}
	\includegraphics[width=0.46\textwidth]{ch10/meankm}
	\end{center}
	\caption{(Color online) \textcolor{red}{Plots cleaned need to be drown nicely}Mean kaons multiplicity produced in p+p interactions as function of collision energy. Statistical uncertainties and systematic uncertainties of \NASixtyOne measurements are presented by lines and shadow band, respectively. Black empty triangles represent the compilation of world data, fully corrected for different effects~{\cite{Anticic:2010yg}}. Magenta empty squares came from Gazdzicki et al.~{\cite{Gazdzicki:1996pk}}. Empty black squares are based on the parametrisation of the old bubble chamber data with statistical error of $20-70\%$~{\cite{Bachler:1999hu,Verbeure:1991tv,Rossi:1974if,Golokhvastov:2001ei,Becattini:1997rv,Back:2003xk}}.}
	\label{fig:Kaonmeanmult}
\end{figure}
 
 Ratio of mean multiplicities of positive and negative kaons produced in protons interactions decreases with the collision energy, and around 40\GeVc $({\sqrt{S_{NN}}=8.8~GeV})$ stabilize to the constant value. It is presented in Fig.~\ref{fig:meankaonsratio} together with the available world data~\cite{Anticic:2010yg}.
  
   \begin{figure}[!ht]
 	\begin{center}
 	\includegraphics[width=0.46\textwidth]{ch10/ratioka}
 	\end{center}
 	\caption{(Color online) Ratio of mean charged kaons multiplicities as function of collision energy.}
 	\label{fig:meankaonsratio}
 \end{figure}
 
The \NASixtyOne measurements allow to study pions production properties. Dependence of the mean negatively and positively charged pions produced per an inelastic event is shown in Fig.~\ref{fig:pionmeanmult}. It can be seen, that $\left\langle\pi^{-/+}\right\rangle$ increases smoothly with the collision energy.
 
\begin{figure}[!ht]
	\begin{center}
	\includegraphics[width=0.46\textwidth]{ch10/meanpip}
	\includegraphics[width=0.46\textwidth]{ch10/meanpim}
	\end{center}
	\caption{(Color online) Mean pions multiplicity as the function of the collision energy. Black empty triangles represents the world data~\cite{Gazdzicki:1995zs}.}
	\label{fig:pionmeanmult}
\end{figure}

 \begin{figure}[!ht]
 	\begin{center}
 	\includegraphics[width=0.46\textwidth]{ch10/ratiopi}
 	\end{center}
 	\caption{(Color online) Ratio of $\left\langle \pi^{+}\right\rangle / \left\langle \pi^{-}\right\rangle$ multiplicities in p+p interactions as the function of the collision energy. World data is presented without uncertainties, thus the plot is more readable.}
 	\label{fig:meanpionsratio}
 \end{figure}
 
 Ratio of mean charged pions multiplicities is presented in Fig.~\ref{fig:meanpionsratio}. It can be observed that at SPS energies range, $\left\langle \pi^{+}\right\rangle / \left\langle \pi^{-}\right\rangle$ ratio slowly decreases with the collision energy. The \NASixtyOne results are in the agreement with other experiments data. 

==> sections/09-onset.tex <==
\section{Energy and system size dependence of particle production}
\label{sec:onset}

%----------------------------------------------------------------------------------------



%%\FloatBarrier
%\subsection{Transverse flow in $p+p$ and $Pb+Pb$ interactions at $158A\ GeV/c$}
%
%Spectra of transverse mass ($m_T$) of negatively and positively charged pions, kaons, protons and $\Lambda$ hyperons~\cite{AWthesis} produced in inelastic $p+p$ interactions at $158~GeV/c$ at mid-rapidity are presented in Fig.~\ref{fig:blast} (left panel). The corresponding data for central $Pb+Pb$ collisions measured by the NA49 experiment~\cite{Alt:2006dk,Alt:2007aa,Afanasiev:2002mx} are shown in the right panel of Fig.~\ref{fig:blast}. These data were fitted using the simplified blast wave model parameterization~\cite{Schnedermann:1993ws}:
%\begin{equation}
%\frac{dN_{i}}{m_{T}dm_{T}dy} = A_{i}m_{T}K_{1}(\frac{m_{T}cosh\rho}{T})I_{0}(\frac{p_{T}sinh\rho}{T}) .
%\end{equation}
%The transverse flow velocity  $\beta_{T}$ was calculated from the equation:
%\begin{equation}
%\rho = \operatorname{tanh}^{-1}\beta_{T}. 
%\end{equation}
%
%\begin{figure}[!ht]
%	\begin{center}
%	\includegraphics[width=0.21\textwidth]{ch10/img/blast_pp}
%   	\includegraphics[width=0.21\textwidth]{ch10/img/blast_PbPb}
%	\end{center}
%	\caption{(Color online) Scaled transverse mass spectra at mid-rapidity measured by the NA61/SHINE experiment in inelastic $p+p$ interactions (left panel) and corresponding results of NA49~{\cite{Alt:2006dk,Alt:2007aa,Afanasiev:2002mx}} from central $Pb+Pb$ collisions at $158A~GeV/c$ (right panel).}
%	\label{fig:blast}
%\end{figure}
%
%The shape of distribution is modified by the transverse flow and presented by the change of $\beta_{T}$ value (see Table~\ref{tab:blast}). The value of $\beta_{T}$ is much higher in central $Pb+Pb$ collisions, than in $p+p$ reactions.
%
%	\begin{table}[!ht]
%%	\resizebox{\textwidth}{!}{
%	\begin{center}
%	\begin{tabular}{ c || c | c }
%    Parameter & $p+p$  & $Pb+Pb$ \\
%	\hline
%	\hline
%	$T\ [MeV]$ & $123\pm1$ & $121\pm1$ \\
%	$\beta_{T}$ & $0.09\pm0.02$ & $0.39\pm0.01$ \\
%	\hline
%	\end{tabular}
%	\end{center}
%%	}
%	\caption{(Color online) Calculated blast wave fit parameters in $p+p$ and $Pb+Pb$ interaction at $158A\ GeV/c$ .}
%	\label{tab:blast}
%	\end{table}	
%
%%%\FloatBarrier
\section{Study of the onset of deconfinement and theoretical models}

%\subsection{Rapidity width of $\pi^{-}$ spectra - dale}
%
%Rapidity distributions of $\pi^{-}$ produced in inelastic $p+p$ collisions~\cite{Abgrall:2013qoa} and energy dependence of the width ($\sigma$) of the rapidity distribution divided by beam rapidity ($\sigma/y_{beam}$) or by the hydrodynamic model prediction ($\sigma/\sigma_{LS}$)~\cite{Landau:1953gs,Shuryak:1974zc} are presented in Fig.~\ref{fig:pimirapidity}. The shape of the rapidity distribution is approximately Gaussian, however the best fit was obtained by a sum of two Gaussian distributions. It can be seen that $\sigma/y_{beam}$ decreases with the collision energy and the values of $\sigma/\sigma_{LS}$ and $\sigma/y_{beam}$ are smaller in $p+p$ than in $Pb+Pb$ interactions. There is not significant difference observed of the energy dependence for the width of the $\pi^{-}$ rapidity distribution in $p+p$ and $Pb+Pb$ interactions. 
%
%\begin{figure*}
%	\begin{center}
%	\includegraphics[width=0.32\textwidth]{ch10/img/rapidity}
%	\includegraphics[width=0.32\textwidth]{ch10/img/sigma_rap}
%	\includegraphics[width=0.32\textwidth]{ch10/img/sigma_La}
%	\end{center}
%	\caption{(Color online) Rapidity distributions of $\pi^{-}$  measured in inelastic $p+p$ collisions at 20, 30.9, 40, 80 and 158~$GeV/c$ (left panel). Dependence of the scaled width of the rapidity distribution of collision energy (middle and right panels) compared with world data~\cite{Klay:2003zf,Abbas:2013bpa,Adler:2003cb}.}
%	\label{fig:pimirapidity}
%\end{figure*}

%%\FloatBarrier
%\subsection{Mean pion multiplicity - kink}
%
%The presented results are an important step towards the study of the system size dependence of signals of the onset of deconfinement observed in central $Pb+Pb$ collisions (kink, horn and step)~\cite{Alt:2007aa,Gazdzicki:2010iv}. The total $\pi$ multiplicity at SPS energies shown in Fig.~\ref{fig:pimimultip} increases faster in the central $Pb+Pb$ than in the inelastic $p+p$ collisions (kink structure). Moreover these two dependencies cross each other at about $40A~GeV/c$.
%
%\begin{figure}[!ht]
%	\begin{center}
%	\includegraphics[width=0.45\textwidth]{ch10/img/kink_zoom}
%	\end{center}
%	\caption{Comparison of the energy dependence of $\pi$ multiplicity for $p+p$ and $Pb+Pb/Au+Au$ interactions.}
%	\label{fig:pimimultip}
%\end{figure}
%%
%%\FloatBarrier
\subsection{Inverse slope parameter of kaons transverse mass spectra - step}

The NA61/SHINE measurements allow to significantly improve the world data on the inverse slope parameter $T$ of transverse mass spectra of kaons~\cite{Kliemant:2003sa} as well as the ratio of $K^+$ and $\pi^+$ yields at the mid-rapidity region~\cite{Gazdzicki:1995zs,Gazdzicki:1996pk}.

Positively and negatively charged kaons spectra at mid-rapidity ($0.0 < y < 0.2$) are shown in Fig.~\ref{fig:kaonsptfinal}. The $p_T$ spectra were parametrized by the exponential function~\cite{Hagedorn:1968jf,Broniowski:2004yh}:
\begin{equation}
%\frac{d^2n}{dp_Tdy}(p_T)_{y}=Ap_Te^{-\frac{\sqrt{p_T^2+m_K^2}}{T}},
 \frac{d^{2}n}{dp_{T}dy}=\frac{S~p_{T}}{T^{2}+m_{K}T}\exp\left(-\frac{\sqrt{p^{2}_{T}+
m^{2}_{K}}-m_{K}}{T}\right),
\label{eq:inverse}
\end{equation}
where: $S$ and $T$ are the yield integral and  the inverse slope parameter, respectively. For better separation, spectra were scaled by the appropriate factors. Shadow bands correspond to systematic uncertainty of the measurements.
	
	\begin{figure}[!ht]
		\begin{center}
		\includegraphics[width=0.2\textwidth]{ch10/Kp_fit_l}
		\includegraphics[width=0.2\textwidth]{ch10/Km_fit_l}
		\end{center}
		\caption{(Color online) Transverse momentum spectra of $K^{+}$ and $K^{-}$ mesons produced at $y\approx 0$ in inelastic $p+p$ interactions
measured by the NA61/SHINE experiment. Color lines represent fitted function (Eq.~{\ref{eq:inverse}}).}
		\label{fig:kaonsptfinal}
	\end{figure}

Figure~\ref{fig:step} presents the energy dependence of the inverse slope parameter $T$ of kaons (step structure). Surprisingly the NA61/SHINE results from inelastic $p+p$ collisions exhibit rapid changes like observed in central $Pb+Pb$ interactions.


\begin{figure*}[!ht]
	\begin{center}
	\includegraphics[width=0.48\textwidth]{ch10/img/stepKM}
	\includegraphics[width=0.48\textwidth]{ch10/img/stepKP}
	\end{center}
	\caption{(Color online) Energy dependence of the inverse slope parameter $T$ of transverse mass spectra of kaons for inelastic $p+p$ interactions and central $Pb+Pb/Au+Au$ collisions~{\cite{Kliemant:2003sa,Abelev:2008ab,Abelev:2014laa,Aamodt:2011zj}}.}
	\label{fig:step}
\end{figure*}

%%\FloatBarrier
\subsection{Kaons to pions ratio - horn}
The acceptance of the identification methods used by NA61/SHINE does not allow to measure spectra
of positive pions close to mid-rapidity region.
Negatively charged pion spectra were obtained by NA61/SHINE in positive hemisphere using the $h^-$ method.
However this method cannot be used for positively charged pions due to the huge contribution of
protons and positive kaons.

Therefore, in order to determine the mid-rapidity yield of positively charged pions,
the following procedure was used:
\begin{itemize}

\item
the $\left\langle\pi+\right\rangle/\left\langle\pi^{-}\right\rangle$ yields were calculated (within the acceptance
of the $tof-dE/dx$ and $dE/dx$ methods) and compared with EPOS model~\cite{Pierog:2009zt} predictions as a function of collision energy (see Fig.~\ref{fig:acceptance}) with the agreement better than $0.1\%$,

\item
the mid-rapidity ratio of the $\pi^+$ and $\pi^-$ yields was calculated from the EPOS model,

\item the $\pi^+$ mid-rapidity yield was calculated as the product of the
measured $\pi^-$ yield (from $h^{-}$ method) at $y=0$, the measured $\frac{\pi+}{\pi^{-}}$ ratio in the $tof-dE/dx$ acceptance and applying the EPOS correction factor:
\begin{equation}
\pi^{+}\left(y=0\right)=\pi^{-}\left(y=0\right) \frac{\pi^{+}}{\pi^{-}}\left(tof-dE/dx\right)C_{MC},
\end{equation}
where:
\begin{equation}
C_{MC}=\left[\frac{\frac{\pi^{+}}{\pi^{-}}(y=0)} {\frac{\pi^{+}}{\pi^{-}}\left(tof\right)}\right]_{MC}\approx 5\%.
\label{eq:CMC}
\end{equation}
\end{itemize}
The obtained values of the correction factor are presented in Fig.~\ref{fig:acceptance}.

\begin{figure*}
	\begin{center}
	\includegraphics[width=0.44\textwidth]{ch10/img/comp_model_tri}
%	\includegraphics[width=0.44\textwidth]{ch10/img/correction}
	\end{center}
	\caption{(Color online) The $\left\langle\pi+\right\rangle/\left\langle\pi^{-}\right\rangle$ in inelastic $p+p$ interactions calculated in the acceptance of the $tof-dE/dx$ and $dE/dx$ identification methods. The NA61/SHINE results are compared to predictions of the EPOS model. }%(left panel). The correction factor used to obtain $\pi^{+}$ yields from the measured $\pi^{-}$ yields is presented in right panel. }
	\label{fig:acceptance}
\end{figure*}

Further study of the phase transition between hadron gas and quark-gluon plasma requires investigation of the strangeness to entropy ratio. This can be realized by study the ratio of koans to pions. The energy dependence of the $K^+ / \pi^+ $ and $K^- / \pi^- $ ratios at mid-rapidity for inelastic $p+p$ interactions and central $Pb+Pb/Au+Au$ collisions are presented in Fig.~\ref{fig:horn}. The NA61/SHINE data suggest that even in inelastic
$p+p$ interactions the energy dependence of the $K^+ / \pi^+$ ratio exhibits rapid changes in the SPS energy range. However, the horn structure is significantly reduced/modified in comparison to that observed in central $Pb+Pb$ collisions. In the Fig.~\ref{fig:horn} also the world data~\cite{Gazdzicki:1995zs,Gazdzicki:1996pk,Arsene:2005mr,Aamodt:2011zj,Abelev:2012wca} is plotted to present the global trend outside the SPS energy range. 

The NA61/SHINE results were compared with theoretical models predictions~\cite{Vovchenko:2014ssa}, namely with EPOS~\cite{Pierog:2009zt}, UrQMD~\cite{Bleicher:1999xi,Bass:1998ca}, Pythia 8~\cite{Sjostrand:2014zea} and HSD~\cite{Ehehalt:1996uq}. It can be concluded that these models models do not describe well the NA61/SHINE results on $p+p$ interactions (see Fig.~\ref{fig:hornModels}). However, high precision of NA61/SHINE data should result in significant improvement of models.

\begin{figure*}
	\begin{center}
	\includegraphics[width=0.48\textwidth]{ch10/img/hornKP}
	\includegraphics[width=0.48\textwidth]{ch10/img/hornKM}
	\end{center}
	\caption{(Color online) The $K^{+}/\pi^{+}$ and $K^{-}/\pi^{-}$ ratios in inelastic $p+p$ and central $Pb+Pb/Au+Au$ reactions for different experimental data.}
	\label{fig:horn}
\end{figure*}

\begin{figure*}
	\begin{center}
	\includegraphics[width=0.48\textwidth]{ch10/img/Kplus_model}
	\includegraphics[width=0.48\textwidth]{ch10/img/Kminus_model}
	\end{center}
	\caption{(Color online) Comparison of $K^{+/-}/\pi^{+/-}$ ratios in inelastic $p+p$ collisions at SPS energies with theoretical models.}
	\label{fig:hornModels}
\end{figure*}

%\FloatBarrier
%\section{Mean transverse mass of protons}
%
%Proton transverse momentum spectra and mean proton transverse mass $\langle m_{T} \rangle$, around mid-rapidity, in inelastic $p+p$ interactions at SPS energies were also study. The results are presented, and compared with theoretical models, in Fig.~\ref{fig:protons}.  Mean $m_{T}$ of protons was calculated from the data parametrization according to
%\begin{equation}
%\frac{d^{2}n}{dp_{T}dy}=\frac{S~p_{T}}{T^{2}+m_{p}T}\exp\left(-\frac{\sqrt{p^{2}_{T}+
%m^{2}_{p}}-m_{p}}{T}\right).
%\end{equation}
%It exhibits a slow increase with the collision energy in contradiction to the UrQMD or HSD models predictions~\cite{Vovchenko:2014ssa}.
%
%\begin{figure}[!ht]
%	\begin{center}
%	\includegraphics[width=0.4\textwidth,valign=c]{ch10/img/pr_pr_fit}
%	\includegraphics[width=0.4\textwidth,valign=c]{ch10/img/mean_mt}
%	\end{center}
%	\caption{(Color online) Proton transverse momentum spectra (left panel) and mean transverse mass $m_{T}$ (right panel), around mid-rapidity, in inelastic $p+p$ interactions at SPS energies compared with theoretical models.}
%	\label{fig:protons}
%\end{figure}
%
%Presented results show that $p+p$ collisions are unexpectedly interesting. Their suggest that even in inelastic $p+p$ interactions the energy dependence of the $K^+ / \pi^+$ ratio and the inverse slope parameter of kaon transverse mass spectra ($T$) exhibits rapid changes in the SPS energy range. However, the structures, e.g. the step and horn, are significantly reduced/modified in comparison to those observed in central $Pb+Pb$ collisions. Understanding and explanation of this behavior is a new puzzle in heavy ion physics. The current level of knowledge and theoretical calculations based on the statistical models, with exact strangeness conservation, suggest that even in $p+p$ collisions we deal with the phase transition~\cite{Poberezhnyuk:2015wea}. %An alternative theory explain observed behavior as associated with the threshold and isospin effects~\cite{Rybicki:2004jd}. Finally it can be concluded that new high precision NA61/SHINE results present challenges for models and should allow for their improvement.

